Linking Aneurysmal Geometry and Hemodynamics Using Computational Fluid Dynamics

The development and progression of abdominal aortic aneurysms (AAA) are related to complex flow patterns and wall-shear-driven mechanobiological stimuli, yet the quantitative relationship between aneurysmal geometry and hemodynamics remains poorly defined. In this study, we conducted a comprehensive hemodynamic analysis of 74 patient-specific abdominal aortas, representing one of the largest Computational Fluid Dynamics (CFD) cohorts reported to date. A multiscale framework coupling 0D-1D systemic circulation models with 3D stabilized finite-element simulations is used to generate physiologically consistent boundary conditions and high-fidelity flow fields. From each model, we extract Time Averaged Wall Shear Stress (TAWSS), Oscillatory Shear Index (OSI), Relative Residence Time (RRT) and Local Normalized Helicity (LNH) indicators alongside an extended set of geometric descriptors characterizing diameter, curvature and torsion. This study provides a clear and comprehensive view of how aneurysm shape influences blood-flow behavior, supported by one of the largest systematically analyzed CFD datasets of AAAs to date. Our results show that specific geometric features reliably shape shear-stress patterns, suggesting that these geometry-driven flow signatures could serve as valuable biomarkers for patient-specific risk assessment. Together, these insights highlight the potential of incorporating detailed geometric descriptors into future models that aim to predict AAA growth and rupture.

==> Figures_Stastics/old_text_statistical_analysis.tex <==
\subsection{Statistical Analysis}
The CFD simulations provided hemodynamic data, including velocity and pressure fields. Critical indices are derived and examined to recognize patterns in our dataset and evaluate the conditions of the patient.

Despite the hemodynamic parameters evaluated in the subsection above, it is crucial to evaluate geometrical characteristics as well. Since each AAA model is unique per patient, geometrical parameters such as the maximum diameter, $d_{max}$, curvature, $\kappa$ and torsion, $\tau$ provided critical information about the variety in aorta models. These parameters were obtained from the centerline of each model using the open source software VMTK~\cite{antiga2008image}.

Statistical analysis was implemented in this section, utilizing in-house codes developed in Matlab. The maximum and mean values of the TAWSS, OSI and RRT were correlated with geometric parameters such as the maximum and mean of the maximum radius, the curvature, as well as the torsion. These geometric parameters were obtained by an in-house Python script that calls via bash scripts the open source software VMTK. By providing the geometry of the CFD simulations to the VMTK, the centerline of each geometry was extracted along with the aforementioned geometric parameters. 

In total, seventy-four $(74)$ AAA models were examined and geometric parameters were extracted. This section aims to statistically correlate the hemodynamic with the geometrical parameters of the models. To generate robust results, the AAA models were divided into two regions: the infrarenal and iliac regions. The Spearman correlation was utilized for each case. Each one of the geometrical parameters was calculated separately for each region. 

The statistical analysis yielded interesting results. More specifically, in Figure \ref{Heatmaps} the heatmaps of the Spearman correlations are displayed, for the infrarenal and iliac regions, respectively. The statistical significance has been set to three cases, $<0.05$, $<0.01$ and $<0.001$. The stars in Figure \ref{Heatmaps} indicate the $p$-value, one star corresponds to $p$-value $<0.05$, two stars to $<0.01$ and three stars to $<0.001$. 

%The most statistically correlated dataset, for the infrarenal part, is the relation between the mean diameter and the mean TAWSS, while the maximum diameter with the mean TAWSS and the mean diameter with the mean RRT give the second most statistically correlated datasets. Lastly, for the infrarenal part, the correlation between the maximum diameter and the mean OSI, the mean diameter and the mean OSI and the maximum diameter and the mean RRT showcased the lower statistically significant correlation. For the iliacs part the results are significantly different since there are more statistically significant correlated datasets with even higher correlation coefficient. 

For the infrarenal part, the mean TAWSS is negatively correlated with the maximum and mean diameter, with coefficients of $\rho=-0.5$ and $\rho=-0.6$, respectively. In both correlations, the $p$-value is $<0.001$, indicating a very strong statistical significance. The mean OSI has also been negatively correlated with the maximum and mean diameter with coefficients of $\rho=-0.24$ and $\rho=-0.29$, respectively. The $p$-value in both correlations was $<0.05$, passing the statistical significance criterion. Lastly, the mean RRT is positively correlated with the maximum and mean diameter with coefficients of $\rho=0.24$ and $\rho=0.31$. It should be noted that for the correlation between the mean RRT and maximum diameter, the $p$-value is $<0.05$ whereas for the correlation between the mean RRT and mean diameters is $<0.01$. 

For the iliac region, a negative correlation is found between the mean diameter and the mean TAWSS with $\rho=-0.94$ and p-value$<0.001$, which is the strongest for the current statistical analysis. In general, for the iliac part, the mean diameter showcased a great correlation between the various hemodynamic parameter. More specifically, the correlation between the mean diameter with the maximum and mean TAWSS results in $\rho=-0.81$ and $\rho=-0.94$, with the maximum and mean OSI results in $\rho=0.41$ and $\rho=0.83$ and finally with the maximum and mean RRT results in $\rho=0.48$ and $\rho=0.89$ respectively. In all of the aforementioned correlations, the p-value is $<0.001$. The maximum diameter showcased a correlation between all of the hemodynamic parameters except the maximum OSI. The maximum diameter correlated with the maximum and mean TAWSS indicates a $\rho=-0.28$ and $\rho=-0.35$ with p-value $<0.05$ and $<0.01$, with the mean OSI $\rho=0.33$ with p-value $<0.01$ and with the maximum and mean RRT $\rho=0.24$ and $\rho=0.35$ with $<0.05$ and $<0.01$, respectively. A special correlation is observed with the maximum curvature with the maximum TAWSS with $\rho=0.32$ and p-value $<0.01$, whereas with the mean TAWSS yield $\rho=0.28$ with $p$-value $<0.05$. Similarly, the correlation of the mean curvature with the mean TAWSS showcase $\rho=0.28$ with $p$-value $<0.05$.

In summary, the splitting of the abdominal aorta into infrarenal and iliac part resulted in different correlations between the geometrical and hemodynamic parameters. In the infrarenal part, the most influential geometrical parameter is the diameter, which is especially correlated with the TAWSS. Similarly, in the iliac part, the diameter has a crucial role in the hemodynamics, whereas the curvature of the iliac also influences these parameters.

Figure \ref{Regression} presents the regression plots for the three most correlated datasets for each of the infrarenal and iliac parts, respectively. In agreement with the previous results from Figure \ref{Heatmaps}, the $R^2$ for the cases of the iliac case showcased better fitting with the datasets, compared to the infrarenal datasets. For the infrarenal part, approximately 2.5\% of the variability of the mean TAWSS is explained by the mean diameter, whereas only 0.9\% by the maximum diameter. Similarly, only 0.5\% of the variability of mean RRT can be explained by the mean diameter. These small percentages indicate that the hemodynamic parameters are not only associated by the maximum and mean diameter.  For the iliac parts, it is shown that approximately 55\% of the variability in the mean TAWSS and mean RRT can be explained by the mean diameter. This percentage increases to approximately 68\% for the variability of the mean OSI with respect to the mean diameter.

Finally, in Figures \ref{Violin_Geo} and \ref{Violin_Hea}, the violin plots of the geometric and hemodynamic parameters are displayed, along with their mean values of the respective parameter.
%The most statistically significant dataset is between the mean diameter and the mean TAWSS whereas the correlation between the mean diameter and mean RRT, the mean diameter and the mean OSI and the mean mean diameter and maximum TAWSS also yield strong statistical correlation. The dataset of the mean diameter with the maximum RRT also gave strong statistical correlation but with smaller correlation coefficient. The less strongly correlated datasets are the maximum diameter with the mean TAWSS, the maximum diameter with the mean RRT, the maximum curvature with the maximum TAWSS. The least correlated datasets are the maximum diameter with maximum TAWSS, the maximum curvature with the mean TAWSS, the mean curvature with the maximum TAWSS and the maximum diameter with the maximum RRT. In summart the mean diameter is strongly correlated with the mean heamodynamic parameters especially in the iliac parts. The infrarenal parts showed no correlation for the curvature and torsion while the iliacs showcased a correlation between the curvature and the TAWSS.
